Distributed Control of Multiagent Systems under Unknown Persistent Disturbances

This paper focuses on the consensus and formation problems of multiagent systems under unknown persistent disturbances. Specifically, we propose a novel method that combines an existing consensus (or formation) algorithm with a new controller. The new controller has an integral action that produces a control input based on an error signal locally projected onto the column space of the graph Laplacian. This action allows agents to achieve a consensus or a predetermined formation objective under constant or time-varying disturbances. This study has analyzed the stability properties of this architecture and provides several illustrative examples to demonstrate the proposed approach.

==> macro.tex <==
\newfont{\smalll}{cmr8}
\def\ID{\hbox{I\hskip-.1em D}}
%\der\IR{\R}
% \def\IR{{\mbox{\hbox{I\hskip-.1em R}}}}
\def\IR{\mathbb{R}}
\def\IS{\mathbb{S}}
\def\Ir{{\mbox{{\smalll I\hskip-0.1em R}}}}
\def\IS{\hbox{I\hskip-.1em S}}
\def\IC{\hbox{C\hskip-
.5em\raise.5ex\hbox{$\scriptscriptstyle\mid$}}\ }
\def\Ic{\hbox{\smalll C\hskip-
.5em\raise.3ex\hbox{$\scriptscriptstyle\mid$}}\ }
\def\IE{\hbox{I\hskip-.1em E}}
\def\IN{\hbox{I\hskip-.1em N}}
\def\IP{\hbox{I\hskip-.1em P}}
\def\SS{\hbox{S\hskip-.4em S}}
\def\vtdef{ {\hskip 0.2em } _ {=} ^{\triangle } {\hskip 0.2em } }
\def\T={\buildrel {\scriptscriptstyle\triangle} \over =}
\newcommand{\ksum}[1]{\buildrel{\scriptscriptstyle #1}\over\oplus}
\def\open#1{\buildrel{\circ}\over{#1}}
\def\blkdiag{\mathop{\rm block{\scriptstyle -}diag}_
{i=1,2} }
\def\notin{\not\hskip-.0em\in}
\def\Empty{/\hskip-0.65em\odot} %\bigcirc}
\def\Empty{\mbox{\O}}
\def\cont{\mbox{\hskip -1 em\,}}
\def\CA{{\cal A}}
\def\CB{{\cal B}}
\def\CC{{\cal C}}
\def\CD{{\cal D}}
\def\CE{{\cal E}}
\def\CF{{\cal F}}
\def\CG{{\cal G}}
\def\CH{{\cal H}}
\def\CI{{\cal I}}
\def\CJ{{\cal J}}
\def\CK{{\cal K}}
\def\CL{{\cal L}}
\def\CM{{\cal M}}
\def\CN{{\cal N}}
\def\CO{{\cal O}}
\def\CP{{\cal P}}
\def\CQ{{\cal Q}}
\def\CR{{\cal R}}
\def\CS{{\cal S}}
\def\CSx{\CS_x}
\def\CT{{\cal T}}
\def\CU{{\cal U}}
\def\CV{{\cal V}}
\def\CW{{\cal W}}
\def\Cw{\small \CW}
\def\CX{{\cal X}}
\def\CY{{\cal Y}}
\def\CZ{{\cal Z}}
\def\CZx{\CZ_x}
\def\BA{\hbox{\bf A}}
\def\BB{\hbox{\bf B}}
\def\BC{\hbox{\bf C}}
\def\BD{\hbox{\bf D}}
\def\BE{\hbox{\bf E}}
\def\BF{\mbox{\bf F}}
\def\BG{\hbox{\bf G}}
\def\BH{\hbox{\bf H}}
\def\BI{\hbox{\bf I}}
\def\BJ{\hbox{\bf J}}
\def\BK{\hbox{\bf K}}
\def\BL{\hbox{\bf L}}
\def\BM{\hbox{\bf M}}
\def\BN{\hbox{\bf N}}
\def\BO{\hbox{\bf O}}
\def\BP{\hbox{\bf P}}
\def\BQ{\hbox{\bf Q}}
\def\BR{\hbox{\bf R}}
\def\BS{\hbox{\bf S}}
\def\BT{\hbox{\bf T}}
\def\BU{\hbox{\bf U}}
\def\BV{\hbox{\bf V}}
\def\BW{\hbox{\bf W}}
\def\BX{\hbox{\bf X}}
\def\BY{\hbox{\bf Y}}
\def\BZ{\hbox{\bf Z}}
\def\sqr#1#2{{\vcenter{\vbox{\hrule height.#2pt\hbox{\vrule
width.#2pt height#1pt \kern#1pt\vrule width.#2pt}\hrule
height.#2pt}}}}
\def\square{\mathchoice\sqr64\sqr64\sqr33\sqr33}
\def\diag{\mathop{\rm diag}}
\def\inf{\mathop{\rm inf}}
\def\block-diag{\mathop{\rm block{\scriptstyle -}diag}}
\def\limsup{\mathop{\rm lim\ sup}}
\def\liminf{\mathop{\rm lim\ inf}}
\def\pmbb#1{\setbox0=\hbox{#1}\raise 0.5ex\box0}
%\def\Cdot{\pmbb .}
\def\Cdot{\cdot}


\def\a{\alpha}
\def\b{\beta}
\def\e{\varepsilon}
\def\t{\theta}
\def\no{\noindent}
\def\s{\sigma}
\def\v{\vert}     \def\V{\Vert}
\def\ha{\hat A}
\def\l{\lambda}
\def\ckZ{\check Z}
\def\nxn{{n\times n}}
\def\underq{\underline q}
\def\underp{\underline p}
\def\underP{\underline P}
\def\RT{\hbox{\smalll T}}
\def\k{\kappa}
\def\L{\Lambda}
%\def\O{\Omega}
\def\o{\omega}
\def\s{\sigma}
\def\j{\jmath}
\def\g{\gamma}
\def\G{\Gamma}
\def\U{\Upsilon}
\def\D{\Delta}
\def\BD{{\bf \Delta}}
\def\d{\delta}
\def\norm#1{\|#1\|}
\def\onorm#1{|\!|\!|#1|\!|\!|}
\def\viks{\rm \vysmall {s}}
\def\vikm{\rm \vysmall {m}}

\def\tmin{\buildrel{\min}\over{\sim}}
\def\tablerule{\noalign{\hrule}}


\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{propo}{Proposition}[section]
\newtheorem{defintion}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{problem}{Problem}[section]

\newcommand{\vtf}[4]{\left[ \begin{array}{c|c}
#1 & #2 \\ \hline #3 & #4 \end{array}\right]}

\newcommand{\mx}{_{\rm mixed}}
\newcommand{\fra}[2]{\mbox{$\frac{#1}{#2}$}}
\newcommand{\und}[1]{{\underline{#1}}}
\newcommand{\jmap}{:\j\IR\rightarrow\IC^{m\times m}}
\newcommand{\RC}{\IR\rightarrow\IC}
\newcommand{\RR}{\IR\rightarrow\IR}
\newcommand{\map}{:\IR\rightarrow\IR^{m\times m}}
\newcommand{\od}{\"{o}}
\newcommand{\Od}{\"{o}}

\newcommand{\etal}{{\it et al. }}
\newcommand{\bequ}{\begin{eqnarray}}
\newcommand{\eequ}{\end{eqnarray}}
\newcommand{\mT}{^\mathrm{T}}
\newcommand{\pr}{\mathrm{Proj}}
\newcommand{\rom}{\mathrm}
%\newcommand{\beqarray}{\begin{eqnarray}}
%\newcommand{\eeqarray}{\end{eqnarray}}
\newcommand{\Real}{{\mathbb{R}}}
\newcommand{\ra}{\rightarrow}
\newcommand{\nn}{\overline{\mathbb{R}}_+}
\newcommand {\subd}     {_{\rm d}}
\newcommand {\mathcalT} {{\mathcal{T}}}
\newcommand {\teq}      {\triangleq}
\newcommand {\mathcalG} {{\mathcal{G}}}
\newcommand {\sube}     {_{\rm e}}
\newcommand{\inv}{^{-1}}
\newcommand {\mathcalK} {{\mathcal{K}}}
\newcommand {\beq}      {\begin{equation}}
\newcommand {\eeq}      {\end{equation}}
\newcommand {\subu}     {_{\rm u}}
\newcommand {\mathcalD} {{\mathcal{D}}}
\newcommand {\subc}     {_{\rm c}}
\newcommand {\subF}     {_{\rm F}}
\newcommand {\mathcalX} {{\mathcal{X}}}
\newcommand{\Proj}{{\mathrm{Proj}}}
\newcommand{\tr}{{\mathrm{tr}}}
\newcommand {\submin} {_{\mathrm{min}}}
\newcommand {\submax} {_{\mathrm{max}}}
\newcommand{\col}{{\mathrm{col}}}
\newcommand {\mathrmC} {{\mathrm{C}}}
\newcommand{\BIS}{{\mathrm{BIS}}}
\newcommand {\subeff}    {_{\rm eff}}


%\newcommand{\T}{{\mathrm{T}}}


\def\Cone{{\rm C}^1}
\def\Hinf{{\rm H}_{\infty}}
\def\Htwo{\mbox{H}_2}
\def\Ltwo{{\rm L}_2}

\def\IR{{\mathbb R}}
\def\IC{{\mathbb C}}
\def\IE{{\mathbb E}}
\def\IN{{\mathbb N}}
\def\IP{{\mathbb P}}
\def\IS{{\mathbb S}}
\def\IT{{\mathbb T}}



\newcommand{\fb}{\hfill$\square$}
\newcommand{\inter}{\mathop{\cap}}
%\newcommand{\prod}{\mathop{\Pi}}
\newcommand{\union}{\mathop{\cup}}


\renewcommand\theenumi{\roman{enumi}}
\renewcommand\theenumii{\alph{enumii}}
\renewcommand\theenumiii{\arabic{enumiii}}
\renewcommand\theenumiv{\Alph{enumiv}}
\renewcommand\labelenumi{{\it\theenumi)}}
\renewcommand\labelenumii{(\theenumii)}
\renewcommand\labelenumiii{\theenumiii.}
\renewcommand\labelenumiv{\theenumiv.}

%Natasa's definitions

\def\Vs{V_{\rm s}}      %storage function               \Vs
\def\Va{V_{\rm a}}      %available storage              \Va
\def\rc{r_{\rm c}}      %supply rate - continious       \rc
\def\rd{r_{\rm d}}      %supply rate - discrete         \rd
\def\Wc{W_{\rm c}}      %supply rate - continious       \Wc
\def\Wd{W_{\rm d}}      %supply rate - discrete         \Wd

\def\CGc{\CG_{\rm c}}

\def\fc{{f_{\rm c}}}      %input - continuous             \fc
\def\fd{{f_{\rm d}}}      %input - discrete               \fd
\def\Gc{{G_{\rm c}}}      %input - continuous             \Gc
\def\Gd{{G_{\rm d}}}      %input - discrete               \Gd
\def\hc{{h_{\rm c}}}      %input - continuous             \hc
\def\hd{{h_{\rm d}}}      %input - discrete               \hd
\def\Jc{{J_{\rm c}}}      %input - continuous             \Jc
\def\Jd{{J_{\rm d}}}      %input - discrete               \Jd

%  for Controller
\def\fcc{f_{\rm cc}}      %input - continuous             \fcc
\def\fdc{f_{\rm dc}}      %input - discrete             \fdc
\def\Gcc{G_{\rm cc}}      %input - continuous             \Gcc
\def\Gdc{G_{\rm dc}}      %input - discrete               \Gdc
\def\hcc{h_{\rm cc}}      %input - continuous             \hcc
\def\hdc{h_{\rm dc}}      %input - discrete               \hdc
\def\Jcc{J_{\rm cc}}      %input - continuous             \Jcc
\def\Jdc{J_{\rm dc}}      %input - discrete               \Jdc


\def\Qc{Q_{\rm c}}      %input - discrete               \Qc
\def\Rc{R_{\rm c}}      %input - discrete               \Rc
\def\Sc{S_{\rm c}}      %input - discrete               \Sc

\def\Qd{Q_{\rm d}}      %input - discrete               \Qd
\def\Rd{R_{\rm d}}      %input - discrete               \Rd
\def\Sd{S_{\rm d}}      %input - discrete               \Sd

\def\Qcc{Q_{\rm cc}}      %input - discrete               \Qc
\def\Rcc{R_{\rm cc}}      %input - discrete               \Rc
\def\Scc{S_{\rm cc}}      %input - discrete               \Sc

\def\Qdc{Q_{\rm dc}}      %input - discrete               \Qd
\def\Rdc{R_{\rm dc}}      %input - discrete               \Rd
\def\Sdc{S_{\rm dc}}      %input - discrete               \Sd

\def\xc{x_{\rm c}}      %state - controller             \xc
\def\xe{x_{\rm e}}
\def\xci{x_{\rm c0}}
\def\uc{u_{\rm c}}      %input - continuous             \uc
\def\ud{u_{\rm d}}      %input - discrete               \ud
\def\yc{y_{\rm c}}      %output - continuous            \yc
\def\yd{y_{\rm d}}      %output - discrete              \yd

\def\ucc{u_{\rm cc}}    %input - continuous             \ucc
\def\udc{u_{\rm dc}}    %input - discrete               \udc
\def\ycc{y_{\rm cc}}    %output - continuous            \ycc
\def\ydc{y_{\rm dc}}    %output - discrete              \ydc
\def\rcc{r_{\rm cc}}    %supply rate - controller/cont. \rcc
\def\rdc{r_{\rm dc}}    %supply rate - controller/disc. \rdc

% DIMENSIONS
\def\mc{{m_{\rm c}}}      %                               \mc
\def\md{{m_{\rm d}}}      %                               \md
\def\lc{{l_{\rm c}}}      %                               \lc
\def\ld{{l_{\rm d}}}      %                               \ld
\def\pc{{p_{\rm c}}}      %                               \pc
\def\pd{{p_{\rm d}}}      %                               \pd

\def\mcc{m_{\rm cc}}      %                               \mc
\def\mdc{m_{\rm dc}}      %                               \md
\def\lcc{l_{\rm cc}}      %                               \lc
\def\ldc{l_{\rm dc}}      %                               \ld
\def\pcc{p_{\rm cc}}      %                               \pc
\def\pdc{p_{\rm dc}}      %                               \pd
\def\kapad{\kappa_{\rm d}}      %                               \pd
\def\kapac{\kappa_{\rm c}}      %                               \pd
\def\nc{n_{\rm c}}      %                               \nc

\def\Vr{V_{\rm r}}
\def\Vsc{V_{\rm sc}}

\def\CUc{\CU_{\rm c}}
\def\CUd{\CU_{\rm d}}
\def\Uc{U_{\rm c}}
\def\Ud{U_{\rm d}}

\def\CYc{\CY_{\rm c}}
\def\CYd{\CY_{\rm d}}
\def\Yc{Y_{\rm c}}
\def\Yd{Y_{\rm d}}

\def\CUcc{\CU_{\rm cc}}
\def\CUdc{\CU_{\rm dc}}

\def\CYcc{\CY_{\rm cc}}
\def\CYdc{\CY_{\rm dc}}
\def\sc{s_{\rm c}}

\def\CTc{\CT^{\rm c}}
\def\CTcc{\CT^{\rm c}_{\rm c}}
\def\CTcon{\CT_{\rm c}}

\def\CTcl{\tilde\CT}
\def\CTclc{\tilde\CT^{\rm c}}

\def\Ad{A_{\rm d}}
\def\Ac{A_{\rm c}}
\def\Bd{B_{\rm d}}
\def\Bc{B_{\rm c}}
\def\Cd{C_{\rm d}}
\def\Cc{C_{\rm c}}
\def\Dd{D_{\rm d}}
\def\Dc{D_{\rm c}}


\def\scq{s_{{\rm c}q}}
\def\fdq{f_{{\rm d}q}}
\def\fcq{f_{{\rm c}q}}
\def\IRc{{\overline{\IR}}}

\def\qc{q_{\rm c}}
\def\rc{r_{\rm c}}
\def\qd{q_{\rm d}}
\def\rd{r_{\rm d}}
\def\elc{\ell_{\rm c}}
\def\eld{\ell_{\rm d}}
\def\CWc{\CW_{\rm c}}
\def\CWd{\CW_{\rm d}}
\def\dc{d_{\rm c}}
\def\dd{d_{\rm d}}
\def\dcr{d_{\rm cr}}
\def\ddr{d_{\rm dr}}
\def\fcr{f_{\rm cr}}
\def\fdr{f_{\rm dr}}
\def\hcr{h_{\rm cr}}
\def\hdr{h_{\rm dr}}
\def\Gcr{G_{\rm cr}}
\def\Gdr{G_{\rm dr}}
\def\Jcr{J_{\rm cr}}
\def\Jdr{J_{\rm dr}}

\def\sc{s_{\rm c}}
\def\sd{s_{\rm d}}


%\newenvironment{proof}{{\bf Proof.}}{\hfill$\square$}

